Geometrical frustration versus Kitaev interactions in BaCo$_2$(AsO$_4$)$_2$

Recently, Co-based honeycomb magnets have been proposed as promising candidate materials to host the Kitaev spin liquid state. One of the front-runners is BaCo$_2$(AsO$_4$)$_2$ (BCAO), where it was suggested that the exchange processes between Co$^{2+}$ ions via the surrounding edge-sharing oxygen octahedra could give rise to bond-dependent Kitaev interactions. In this work, we present and analyze comprehensive inelastic neutron scattering studies of BCAO with fields in the honeycomb plane. Combining the constraints from the magnon excitations in the high-field polarized state and the inelastic spin structure factor measured in zero magnetic field, we examine two leading theoretical models: the Kitaev-type \JKG model and the \XXZ model. We show that the existing experimental data can be consistently accounted for by the \XXZ model but not by the \JKG model, and we discuss the implications of these results for the realization of a spin liquid phase in BCAO and more generally for the realization of the Kitaev model in cobaltates.

==> discussion_v2.tex <==
Though our initial interest in BCAO was as a candidate Kitaev material, our results strongly favor the \XXZ model over the Kitaev case. Firstly, we are able to differentiate between the two models by examining the zero-field ground state of BCAO. We find that the \JKG model cannot reproduce the field dependence of the dispersion at the $\Gamma$-point and the right classical ground state. The incommensurate spiral order reported for BCAO is also incompatible with a large ferromagnetic Kitaev interaction, even with the addition of third nearest neighbor interaction. On the other hand, such a magnetic order is reproduced in the \XXZ picture. Perhaps the most striking contrast between the two models is seen in our DSSF results presented in Fig. \ref{fig:dssf_md_fig}. Qualitatively, it is immediately obvious that the \JKG model fails to describe the zero-field INS, whereas the \XXZ model is able to capture some highly non-trivial features especially at high temperature. Lastly, the in-plane magnetization curves predicted by the \XXZ model at finite temperature is in remarkable qualitative agreement with measurements and can even reproduce subtle features such as small anistropy observed between different field directions. The \JKG model, however, yields highly anisotropic curves, which further supports the \XXZ picture as a description for BCAO. In conclusion, our work provides compelling evidence for the description of BCAO in terms of an \XXZ model with only small bond dependant interactions as it is able to reproduce many non-trivial measurements, whereas the \JKG model cannot account for these observations. Furthermore, we provide hard constraints on possible microscopic couplings for this model, making BCAO amenable to meaningful and specific future theoretical predictions.

Our work stresses the necessity of a critical reexamination of the proposal for Kitaev physics in cobaltates. Indeed, our results combined with the \emph{ab initio} study \cite{Das2021XYCobaltates} indicates that the weak spin-orbit coupling of Co$^{2+}$ makes the mechanism proposed in \cite{Liu2018PseudospinModel, Sano2018Kitaev-HeisenbergInsulators} to generate a large Kitaev interactions extremely sensitive to local distortions of the crystal field environment, which are unavoidable in real materials. It is also likely that many cobaltates do not fall within the regime of interest that was considered in these theoretical proposals where direct hopping was assumed to be much weaker than ligand-assisted hopping, and further neighbor interaction altogether neglected. We therefore emphasize the need for thorough \emph{ab initio} examination of the exchange interactions of other cobaltates that were proposed as KSL candidates, and underscore the great caution required to interpret future results before making any claim about the apparent realization of Kitaev physics. As an example, by simply fitting the INS spectrum of BCAO along the $(h00)$ direction in the polarized regime, one could have wrongly reached the conclusion that the low energy physics could be modelled by a large ferromagnetic Kitaev interaction with subdominant isotropic and off-diagonal interaction as in Eq. \eqref{eq: representative points JKGGp}. It is therefore imperative to ensure that the proposed model is compatible with the observed ground state order and thermodynamics measurements. Examples of potential materials that fit this call for the reassessment of magnetic interactions in honeycomb cobaltates are Na$_2$Co$_2$TeO$_6$ \cite{Yao2020FerrimagnetismNa2Co2TeO6}, Li$_3$Co$_2$SbO$_6$ \cite{Vivanco2020CompetingMagnet}, and Na$_3$Co$_2$SbO$_6$ \cite{Songvilay2020KitaevNa2Co2TeO6}, which all feature strongly easy-plane anisotropy and curious field-driven transitions \cite{Yao2020FerrimagnetismNa2Co2TeO6} similar to BCAO. \THComment{ Add more references here. } 


As experimentally relevant methods for this critical reexamination of cobaltates, we suggest the investigation of angle-dependant magnetization and specific heat. Indeed, the \JKG model with large Kitaev interaction generically predicts significant anisotropy for thermodynamic quantities as a function of an in-plane field angle (e.g., see fig. \ref{fig:md_magnetization}) in opposition to the \XXZ model that only produces isotropic response for in-plane probes. As a matter of fact, such anisotropic behavior has been observed in the leading Kitaev candidate $\alpha$-RuCl$_3$  \cite{Bachus2021Angle-dependent-RuCl3,Tanaka2022ThermodynamicLiquid} as well as in $\beta-$Li$_2$IrO$_3$ \cite{Majumder2019AnisotropicStudy}. Such simple methods are of great practical interest since they avoid more challenging techniques like single crystal INS. For candidate cobaltates whose behavior could not be explained by the \XXZ or other simple model, single crystal INS examining the polarized states of these materials may be necessary to unambiguously reveal the nature of their magnetic interactions. 


Although BCAO does not appear to host large Kitaev-type interactions, the \XXZ model is nonetheless still of great interest. The geometric frustration due to the competition between first and third nearest neighbor could potentially imply that BCAO is in close proximity to a QSL. Point in fact, previous theoretical investigations have demonstrated the possibility of purely isotropic models on the honeycomb lattice to host QSLs ground states \cite{merino2018role, zhu2014quantum, bishop2012frustrated}. Although all of these studies have reported the necessity of second nearest-neighbor interaction (which seems to be negligible for BCAO) to stabilize a QSL, it might still be conceivable to drive an XXZ system in close proximity to a QSL by applying an external magnetic field. Such a possibility has, to our knowledge, not been explored yet. The spectral weight collapse with the application of an out-of-plane field reported by THz spectroscopy \cite{Zhang2021In-BaCo_2AsO_4_2} may potentially signal the onset of such a topological phase. %We leave this work for future studies, but this seems to be the most 
\EZchange{This work is a }promising direction for \EZchange{future studies} of BCAO and a number of other existing honeycomb cobaltates.


\emph{Note added:} While writing this paper, we became aware of three \emph{ab initio} theoretical investigations of BCAO. Two of them \cite{maksimov2022ab, winter2022magnetic} corroborate our conclusion regarding the nature of magnetic interaction in BCAO and propose a coherent microscopic theory for it. On the contrary, one \cite{Samantha2022} claims to observe the formation of spin-orbit-entangled $J_{eff}$=1/2 moments that could potentially support the claim of Kitaev physics. The former two importantly find that the double-zigzag state is not stabilized classically, even if it is energetically proximate to the incommensurate spiral phase (just as we do), but can be promoted as the true ground state by quantum fluctuations or relaxation of the atomic positions.

==> intro_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%              Introduction                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
% The Kitaev honeycomb model is an exactly solvable model where spins-1/2 moments are coupled through Ising-like bond dependent interactions that hosts an exotic magnetic ground state known as a quantum spin liquid (QSL) where the spin degrees of freedom remain fluctuating rather than magnetically ordered at T=0 K. 
% The resulting Kitaev spin liquid (KSL) is characterized not simply by a lack of magnetic order but by long-range entanglement that leads to the emergence of exotic excitations such as \mathbb{Z}$_2$ gauge fluxes and Majorana fermions. The Kitaev spin liquid (KSL) is unique in that it is a rare exactly solvable model of a QSL in higher than one dimension with realistic pathways to physical realizations in condensed matter systems. 
% \EZComment{I think the exact solvability isn't really relevant for this paper; it's also mentioned in the first sentence. We can probably cut this sentence.} 

The Kitaev honeycomb model consists of spin-1/2 moments coupled through Ising-like bond-dependent interactions, and hosts an unusual magnetic ground state known as a quantum spin liquid (QSL). The resulting Kitaev spin liquid (KSL) state is characterized by the emergence of exotic excitations such as $\mathbb{Z}_2$ gauge fluxes and Majorana fermions \cite{Kitaev2006AnyonsBeyond,hermanns2018physics,takagi2019concept,balents2010spin,wen2004quantum, savary2016quantum,zhou2017quantum,broholm2020quantum, knolle2019field}. In the majority of proposed candidate Kitaev materials, the chemical mechanism to induce the anisotropic bond-dependent Kitaev interaction relies on exchange processes involving $4d$ and $5d$ systems that have large spin-orbit coupling (SOC) such as Ru$^{3+}$ and Ir$^{4+}$  \cite{Jackeli2009MottModels, Rau2016Spin-OrbitMaterials}. However, in such materials relatively large non-Kitaev interactions induce magnetic order at low temperature and obscure possible signatures of Kitaev physics \cite{Rau2014GenericLimit, Plumb2014-Lattice,Banerjee2017Neutron-RuCl3,Banerjee2018Excitations-RuCl3,Biffin2014UnconventionalDiffraction,Ducatman2018Magnetic-Li2IrO3,Majumder2018Breakdown-Li2IrO3,Takayama2015HyperhoneycombMagnetism}. One is thus left with the hope of potentially driving the system in close proximity to a KSL state by tuning external parameters such as the magnetic field \cite{Banerjee2018Excitations-RuCl3,Zheng2017Gapless-RuCl3,Baek2017Evidence-RuCl3,Kasahara2018MajoranaLiquid}. 


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/structure_figure_2.png}
    \caption{(a) Honeycomb lattice of BCAO viewed along the $c$-axis. Cobalt ions are shown in blue, oxygen in red, and arsenic is in green. The first Brillioun zone of the hexagonal lattice is shown along reciprocal lattice vectors $\textbf{g}_1$ and $\textbf{g}_2$. The high symmetry points $M$ and $K$ are shown using the red and blue squares, respectively. (b) Representation of the XXZ-$J_1$-$J_3$ model. The global Cartesian frame is shown to the right in the black axes. (c) Local spin-frame picture for Kitaev interaction on the honeycomb lattice. The $x$, $y$ and $z$ bonds  are shown in blue, green, and red coloring respectively.} \label{fig:structure_fig}
\end{figure}

A new mechanism for a more ideal material realization of the Kitaev model has recently been put forward for high-spin 3$d^{7}$ cobaltates in the ($S=3/2$ $L=1$) configuration \cite{Liu2018PseudospinModel,Sano2018Kitaev-HeisenbergInsulators}. It was suggested that, in ideal circumstances, various exchange processes involving the $t_{2g}$ and $e_{g}$ orbitals will lead to a dominant ferromagnetic Kitaev interaction between the $J_{eff}=1/2$ pseudospins with only relatively weak non-Kitaev couplings. One of the most promising candidates of such a 3$d^{7}$ Kitaev material is the layered honeycomb magnet BaCo$_2$(AsO$_4$)$_2$ (see Fig. \ref{fig:structure_fig} (a)), hereby referred to as BCAO. Detailed heat capacity, magnetization, and neutron scattering studies have previously observed that BCAO magnetically orders into an incommensurate phase at T$_N$=5.5 K with an ordering wavevector of $\vec{k}_{c}=(0.27,0,-1.31)$. Further, it undergoes two successive phase transitions with an applied in-plane field: first for  $H_{C_{1}}=0.33$~T into a commensurate ordered state with wavevector $\vec{k}_{c}=(1/3,0,-1.31)$, and at a second into a partially field-polarized state at a critical field $H_{C_{2}}=0.55$~T \cite{Zhong2020Weak-fieldHoneycomb, Regnault1977MagneticBaCo2AsO42,Regnault1990PhaseMagnets, Regnault2018Polarized-neutronMagnet}. In light of the new theoretical prediction for Kitaev physics in cobaltates, the observation that the magnetic order could be suppressed with such a small in-plane field led to the proposal of an easily accessible field-induced KSL. Further observations by THz spectroscopy studies of a spectral weight collapse at the $\Gamma$-point \cite{Zhang2021In-BaCo_2AsO_4_2,Shi2021MagneticSpectroscopy} for an out-of-plane field accompanied by the absence of Goldstone mode at the incommensurate ordering wavevector, as already noted by early neutron scattering investigations \cite{Regnault1977MagneticBaCo2AsO42}, generated speculations that BCAO is potentially the most ideal realization of a KSL known up-to-date \cite{Zhang2021In-BaCo_2AsO_4_2}. 

Following the modern proposal of Kitaev physics in BCAO, a follow up ab-initio study suggested an entirely different story \cite{Das2021XYCobaltates}. This investigation reported that the weak SOC in 3$d$ transition metals makes the Kitaev physics in colbatates extremely fragile to the presence of trigonal distortions that were not accounted for in the proposed Co$^{2+}$ Kitaev mechanism. For this reason, BCAO was observed to be better described by an easy-plane XXZ model with significant geometrical frustration coming from large third nearest-neighbor interactions (XXZ-$J_{1}$-$J_{3}$ model). Previous studies on the similar material BaCo$_2$(PO$_4$)$_2$ were able to completely describe the ground state using a very similar model \cite{Nair2018Short-rangeBaCo2PO42}, which also suggests that types of interactions may be manifested in BCAO. 

Little experimental work has been done to distinguish the JK$\Gamma$-$\Gamma'$ model from the XXZ-$J_{1}$-$J_{3}$ model in BCAO and other cobaltates. In this work, we perform two detailed INS experiments, one with zero-field in the $(HK0)$ scattering plane and the other in the $(H0L)$ scattering plane with a field applied along the basal plane. The full magnetic excitation spectra is mapped, allowing for a critical examination of the two competing models. Our results may be summarized in the following way. First, using linear-spin wave theory in the field-polarized regime we tightly constrain where BCAO may lie in parameter space for each model. Then, within this constrained subspace, we examine the magnetic ground states that are realized. While both models accommodate incommensurate magnetic order, the spiral order with ordering wavevector between the $\Gamma$ and M points cannot be stabilized in the Kitaev case. Additionally, we observe that even if both models can reproduce the observed inelastic scattering in the field-polarized state, molecular dynamics (MD) calculations reveal that the dynamical spin-structure factor at zero field seems incompatible with for a model with large ferromagnetic Kitaev interaction, whereas it can be adequately accounted for using an XXZ-$J_{1}$-$J_{3}$ spin Hamiltonian with only weak bond-dependent interactions. Finally, for a properly chosen parameter set, we are able to observe an in-plane magnetization curve with three successive plateaus separated by two field-induced phase transitions with only small anisotropy for different in-plane direction in remarkable qualitative agreement with experimental measurements for the XXZ-$J_{1}$-$J_{3}$. We thus find compelling evidence indicating that BCAO is not a realization of the Kitaev model, but rather a geometrically frustrated easy-plane magnet with predominantly isotropic exchange. 

Our work highlights the need for a more thorough examination of the exchange interactions in the honeycomb cobaltates, a number of which have been proposed as KSL candidates. While a set of exchange parameters with a large Kitaev interaction can reproduce the observed INS excitation spectra with an easily obtained LSWT fit, it should always be verified that this parameter set is consistent with the zero-field ordered state. Even though BCAO does not appear to have strong Kitaev interactions based on our work, it still may be quite close to a QSL driven by geometrical frustration. The emergence of a continuum for an out-of-plane field upon the suppression of order revealed in THz spectroscopy \cite{Zhang2021In-BaCo_2AsO_4_2} might be a signature of such a proximate QSL whose characteristics would most likely differ significantly from the KSL. As a result, we speculate on a potential out-of-plane field-induced QSL using the extracted exchange parameters and propose directions for future works.

